Adaptive Matching for Expert Systems with Uncertain Task Types

A matching in a two-sided market often incurs an externality: a matched resource may become unavailable to the other side of the market, at least for a while. This is especially an issue in online platforms involving human experts as the expert resources are often scarce. The efficient utilization of experts in these platforms is made challenging by the fact that the information available about the parties involved is usually limited. To address this challenge, we develop a model of a task-expert matching system where a task is matched to an expert using not only the prior information about the task but also the feedback obtained from the past matches. In our model the tasks arrive online while the experts are fixed and constrained by a finite service capacity. For this model, we characterize the maximum task resolution throughput a platform can achieve. We show that the natural greedy approaches where each expert is assigned a task most suitable to her skill is suboptimal, as it does not internalize the above externality. We develop a throughput optimal backpressure algorithm which does so by accounting for the `congestion' among different task types. Finally, we validate our model and confirm our theoretical findings with data-driven simulations via logs of Math.StackExchange, a StackOverflow forum dedicated to mathematics.

==> Data.tex <==
% !TEX root = Journal_ExpertSystems.tex


\section{Math.Stack-Exchange Dataset}


We examined the math.stack-exchange Question \& Answer database (version $2$ February $2017$) where users post tagged questions that are answered by other users. The asker may accept one answer that he believes is the best solution to his problem. 

We ranked the different tags according to their occurrence: calculus is most popular ($61184$ questions), while complex analysis ($22813$ questions) is on the $11$-th place. 
We filtered the mathematics database so to have only questions with at least one of the $11$ most popular tags, amounting to a total of $381239$ questions.




\begin{table}
\begin{tabular}{ |c||c||c||c||c||c||c||c||c||c||c|  }
 \hline
 \multicolumn{11}{|c|}{Clusters} \\
 \hline
 \textbf{Tag} & $c_1$ & $c_2$ & $c_3$ & $c_4$ & $c_5$ & $c_6$ & $c_7$ & $c_8$ & $c_9$ & $c_{10}$ \\
 \hline
calculus & .32 & \textbf{.39} &.30 &\textbf{.35} &\textbf{.37} &\textbf{.47} &.28 &.16 &.26 &\textbf{.41} \\
real-analysis & .17 &\textbf{.41} &.25 &.32 &.23 &\textbf{.49} &\textbf{.40} &.10 &.10 &\textbf{.44} \\
linear-algebra &\textbf{.46} &.29 &.05 &\textbf{.36} &.14 &\textbf{.48} &.26 &.31 &.07 &\textbf{.43} \\
probability & .07 &\textbf{.49} &.02 &.33 &.02 &\textbf{.50} &.06 &.02 &\textbf{.46} &.04 \\
abstract-algebra & .02 &.05 &.03 &.32 &.02 &\textbf{.38} &.23 &\textbf{.50} &.01 &.27 \\
integration &.09 &\textbf{.43} &.05 &.19 &\textbf{.44} &\textbf{.45} &.03 &.01 &.06 &\textbf{.37} \\
sequences-and-series &.05 &.32 &.16 &.31 &.20 &\textbf{.45} &.09 &.04 &.06 &.33 \\
general-topology & .02 &.10 &.03 &.16 &.02 &\textbf{.43} &\textbf{.50} &.07 &.02 &.31 \\
combinatorics &.03 &.14 &.06 &\textbf{.43} &.04 &\textbf{.37} &.02 &.06 &.19 &.05 \\
matrices &.27 &.15 &.02 &.31 &.02 &\textbf{.44} &.06 &.11 &.02 &.34 \\
complex-analysis & .02 &.19 &.08 &.16 &.14 &\textbf{.50} &.09 &.05 &.01 &\textbf{.44} \\
 \hline
 \hline
 \textbf{Size} & 165 & 188 & 313 & 200 & 179 & 183 & 231 & 187 & 178 & 176 \\
 \hline
\end{tabular}
 \caption{Demonstration of heterogeneity in experts at Math.Stack-exchange Q\&A platform}
\end{table}



For a given user $u$ and tag $t$, we denote by $n_u^{\text{answers}}(t)$ the number of times $u$ answered to questions of tag $t$ and by $n_u^{\text{accepted}}(t)$ the number of accepted answers among them. We estimate the performance of $u$ on $t$ as
$$
p_u^t = \left\{
    \begin{array}{ll}
        \frac{n_u^{\text{accepted}}(t)}{n_u^{\text{answers}}(t)} & \mbox{if  } n_u^{\text{accepted}}(t) > 5 \\
        0 & \mbox{otherwise.}
    \end{array}
\right.
$$

We calculated the performances of the $2000$ users with the most accepted answers. The top user has $4665$ accepted answers, $712$ users have more than $50$ answers accepted, and the user at place $2000$ has $13$ of his answers accepted. To form groups of users with similar performance over the different tags, we considered the performance vectors $(p_u^{\text{calculus}}, \ldots, p_u^{\text{complex-analysis}})$ of individuals as points in an $11$-dimensional space, and ran k-means on them. 

The result is displayed in Table ??. The columns $c_1, \ldots, c_{10}$ are the centroids of the clusters and give the average performance on the tags. Just below a column, we give the size of the corresponding cluster. For instance, the $165$ persons in $c_1$ have on average $32\%$ of their calculus, and $46\%$ of their linear algebra answers accepted.


We put all scores above $35\%$ in boldface and observed the following heterogeneity: Cluster $c_6$ contains $183$ very active, experienced users doing very well on all tags. Cluster $c_3$ contains the bulk of $313$ users with low performance over all tags. The clusters $c_1, c_7, c_8$ and $c_9$ contain users specialised in a single topic. The users in the remaining clusters $c_2,c_4,c_5$ and $c_{10}$ do well on a few related topics.
  





==> Introduction_old.tex <==
% !TEX root = EC2017_ExpertSystems.tex


\section{Introduction}
\label{sec:intro}

Online platforms that enable matches between trading partners in two-sided matching markets have recently blossomed in many areas: 
%There has been a raise of online platforms that enable transactions between trading partners at an unprecedented scale in a wide-variety of matching markets. 
LinkedIn and Upwork facilitate matches between employers and employees; Uber allows matches between passengers and car drivers; Airbnb and Booking.com connect travellers and housing facilities; Quora and Stack Exchange facilitate matches between questions and  either answers, or experts able to provide them. 

All these systems crucially rely on the ability to propose adequate matches based on imperfect knowledge of the characteristics of the two parties to be matched.
%A key component of all these systems is a matchmaking that is required to be efficient in quickly finding relevant matches and robust to uncertainty of information about features of the potential trading partners. 
For example, in the context of online labour platforms, there is uncertainty about both the skill sets of candidate employees and the job requirements. Similarly, in the context of online Q\&A platforms, there is uncertainty about both question types and users' ability to provide answers. 

This naturally leads to the following question: which matching recommendation algorithms can, in the presence of such uncertainty, lead to efficient platform operation? A natural measure of efficiency is the throughput that the platform achieves, i.e. the rate of successful matches it allows. To address this question, one thus needs first to characterize fundamental limits on the achievable throughput. 

In this paper we progress towards answering these questions as follows. 

First, we propose a simple model of such platforms, which features a static collection of servers, or experts on the one hand, and a continuous stream of arrivals of tasks, or jobs, on the other hand. In our model, the platform's operation consists of servers iteratively attempting to solve tasks. After being processed by some server, a task leaves the system if solved; otherwise it remains till successfully treated by some server. 
To model uncertainty about task types, we assume that for each incoming task we are given the prior distribution of this task's ''true type''. Servers' abilities are then represented via the probability that each server has to solve a task of given type after one attempt at it. 

In a Q\&A platform scenario, tasks are questions, and servers are experts; a server processing a task corresponds to an expert providing an answer to a question. A task being solved corresponds to an answer being accepted. In an online labour platform, tasks could be job offers, and a server may be a pool of workers with similar abilities. A server processing a task then corresponds to a worker being interviewed for a job, and the task is solved if the interview leads to a hire. We could also consider the dual interpretation when the labour market is constrained by workers rather than job offers. Then a task is a worker seeking work, while a server is a pool of employers looking for hires. 

An important feature of our model consists in the fact that when a task's processing does not lead to failure, it does however affect uncertainty about the task's type. Indeed the a posteriori distribution of the task's type after a failed attempt on it by some server differs from its prior distribution.For instance in a Q\&A scenario, a question  which an expert in Calculus failed to answer either is not about Calculus, or is very hard. 

For our model, we then determine necessary and sufficient conditions for an incoming stream of task arrivals to be manageable by the servers, or in other words, what is the achievable throughput of the system. In the process we introduce candidate policies, in particular the greedy policy according to which a server choses to serve on tasks for which its chance of success is highest. This scheduling strategy is both easy to implement and is based on a natural motivation. Surprisingly perhaps, we show that it is not optimal in the throughputs it can handle. In contrast, we introduce a so-called back-pressure policy inspired from the wireless networking literature \cite{TaE92}, which we prove to be thoughput-optimal.

To validate our modeling and theoretical results, we analyse logs from MathOverflow, a StackOverflow forum specializing on mathematics. Our data analysis corroborates several aspects of our model, notably the modeling of uncertainty about task types as a a prior on task type, together with the modeling of server ability through their success probability on each task type. Numerical experiments based on MathOverflow data analysis confirm the theoretical results, namely that our back-pressure policy can achieve significantly higher throughputs than other baseline policies.



%In this paper we study matching of tasks and experts where the types of tasks are uncertain in a system described as follows. Tasks arrive online, each of an unknown type according to a known prior distribution. Each expert attempts to solve tasks at a rate that is allowed to be specific to each given expert. Upon each attempt of an expert solving a task, the task is is successfully resolved with a probability that is allowed to be specific to given expert and the task type. As soon as a task is successfully resolved, it is removed from the system. Upon each unsuccessful attempt by an expert to solve a task, some information is revealed about the task type, which is captured by the posterior distribution of the task type. 

%We model our system dynamics via a Markov chain where given the past and the present, the future events are independent of the past. Unconditionally, however, the future and the past may not be independent. Unlike discrete time models where the system state may change after exactly a unit time, we admit a continuous time Markov chain where the state may change after a random time. Owing to the {\em memoryless} property of the exponential distribution, which allows us to retain the Markov property in continuous time, we let the time between two consecutive task arrivals as well as the response time of an expert to be exponentially distributed, possibly with different rates depending on the expert's speed. 

%The main goal of this paper is to characterize the maximum rate at which tasks can be served by a task-expert system, under which the system is stable, i.e. under which there exists a time-stationary regime under which the expected number of tasks waiting to be served in the system is finite. Stability is important as it implies that each task receives a successful response in a finite expected time. This is a fundamental question that one needs to address before going on to consider various particular policies for matching tasks to experts with the goal to optimize a given objective function, such as minimizing the long-run average of the number of tasks waiting to be served in the system. 

%The model of a task-expert system formulated in this paper formally corresponds to a queueing system, which to the best of our knowledge is different from any previously studied models in queueing theory literature, \eg, see \cite{TaE92,MaS04} and other related works described in Section~\ref{sec:related}. The key difference is the assumption that types of tasks are uncertain, and need to be learned by exploration. Our model is also different from that studied in the context of online stochastic matching, \eg, see \cite{MeP12} and other related works described in Section~\ref{sec:related}, where it is typically assumed that either tasks or experts are offline entities that serve a limited number of assignments. In our case, experts are assumed to be offline entities that recurrently attempt to solve tasks, assigned to them by a matchmaking policy. This amounts to studying the long-run performance of the system in a time-stationary regime, as opposed to studying the performance over a finite time period.   

We summarize contributions of this paper as follows:
\begin{itemize}
\item We propose a new model of a generic task-expert system that allows for uncertainty of task types, heterogeneity of skills, and recurring attempts of experts in solving tasks. 
\item We provide a full characterization of the stability region, or sustainable throughputs, of the task-expert system under consideration. We establish that a particular back-pressure policy is throughput-optimal, in the sense that it supports maximum task arrival rate under which the system is stable.  
\item We show that there exist instances of task-expert systems under which simple matchmaking policies such as a natural greedy policy and a random policy can only support a much smaller maximum task arrival rate, than the back-pressure policy.
\item We report the results of empirical analysis of the popular MathOverflow Q\&A platform which establish heterogeneity of skills of experts, with experts knowledgeable across different types of tasks and others specialized in particular types of tasks. We also show numerical evaluation results that confirm the benefits of the back-pressure policy on greedy and random matchmaking policies.
\end{itemize} 

The remainder of the paper is structured as follows. Section~\ref{sec:system} presents our system model. In Section~\ref{sec:strawman}, we present results for two baseline matchmaking policies, namely  Greedy and Random, and a characterization of achievable throughputs under Random. Section~\ref{sec:stability} presents the characterization of task arrival rates that can be supported under which the system is stable and prove the superiority of back-pressure policy over Random and Greedy. In Section~\ref{sec:exp}, we present our experimental results. Related work is discussed in Section~\ref{sec:related}. We conclude in Section~\ref{sec:conc}. Proofs of the results are provided in the Appendix, added as a supplementary material. 



==> Simulations.tex <==
% !TEX root = EC2017_ExpertSystems.tex


\section{Simulations}




Could start with the following example:

\begin{example}[Anti-symmetric expertise]\label{eg:Antisymmetry}
Suppose $S = \{s_1,s_2\}$,  $C = \{c_1,c_2\}$, $\pi_{z} = 1$ for $z=(0.5,0.5)$, $\mu_s = 1$ for each $s$. Further suppose $p_{s_1}^{c_1} = p_{s_2}^{c_2} \overset{(\text{say})}{=} a $, $p_{s_1}^{c_2} = p_{s_2}^{c_1} \overset{(\text{say})}{=} b$, \ie, the expertise is anti-symmetric. Suppose $a > b$. Then we have stability when $\lambda < 4\frac{a+b-ab}{4-a-b}$ for both greedy and back-pressure.
\end{example}


Other candidate policy we could simulate:

Max-weight:
$$z(s) \in A_s(N) = \arg\min_{z:N_z > 0} \sum_c q_c(N) z_c p_{sc}$$


